ELight: Enabling Efficient Photonic In-Memory Neurocomputing with Life Enhancement

With the recent advances in optical phase change material (PCM), photonic in-memory neurocomputing has demonstrated its superiority in optical neural network (ONN) designs with near-zero static power consumption, time-of-light latency, and compact footprint. However, photonic tensor cores require massive hardware reuse to implement large matrix multiplication due to the limited single-core scale. The resultant large number of PCM writes leads to serious dynamic power and overwhelms the fragile PCM with limited write endurance. In this work, we propose a synergistic optimization framework, ELight, to minimize the overall write efforts for efficient and reliable optical in-memory neurocomputing. We first propose write-aware training to encourage the similarity among weight blocks, and combine it with a post-training optimization method to reduce programming efforts by eliminating redundant writes. Experiments show that ELight can achieve over 20X reduction in the total number of writes and dynamic power with comparable accuracy. With our ELight, photonic in-memory neurocomputing will step forward towards viable applications in machine learning with preserved accuracy, order-of-magnitude longer lifetime, and lower programming energy.

==> doc/5discuss.tex <==
\section{Tolerating Scheme against Aged PCM Wires }
% {Tolerating Aged PCM Wires via Global Row Swapping}
\label{sec:tolerate}
We further equip our framework \texttt{ELight} with a global row-based remapping method to tolerate aged PCM wires inside photonic memories in an efficient way, thus enabling the photonic in-memory neurocomputing with higher resilience against PCM aging issues.

The phase state of aged PCM wires is complex to analyze, causing uncontrolled drifts from desired values.
As not all PCM wires in the memory cells wear out simultaneously, one way to enable further utilization of aged memory cells is to tie the aged wires to known phase states.
Considering a typical bell-shaped distribution with more weights around the mean for neural networks \cite{NN_Arxiv2015_han}, setting aged wires to $c$ state is preferred to ensure the representability of small transmission values.
In this regard, with aged wires within photonic memory cells, their implementable transmission range will degrade, as shown in Fig.~\ref{fig:StruckFaultMapDeviation}. 
As the upper bound $T_{max}$ and the lower bound $T_{min}$ of transmission values decrease in the aged cell,
% if the value range of a sequence of weights exceeds the supported transmission range, 
directly mapping weights, whose range exceeds the supported transmission range, on the aged cell will result in mapping deviation.
The mapping deviation affects the encoded weights and leads to inaccurate calculation, resulting in severe accuracy degradation.
% \JG{Unfortunately, the accuracy of neural networks is very sensitive to value variations, resulting in severe accuracy degradation. }

\begin{figure}
    \centering
    \includegraphics[width=0.38\textwidth]{figs/StruckFaultMapDeviation_v2.pdf}
    \vspace{-5pt}
    \caption{\small~Mapping deviation on aged PCM cells.}
    \label{fig:StruckFaultMapDeviation}
\end{figure}

Thus, to enable tolerance against aged PCM wires, a global row-based remapping method is proposed to reorder the rows of the weight blocks and remap weight blocks to the PTCs to obtain the smallest mapping deviation, shown as phase 3 in Fig.~\ref{fig:ElightFlow}.
Different from previous art~\cite{NP_DATE2017_chen},
we reorder the rows of a group of weight blocks in the same order, benefiting from the block similarity brought by the block matching.
Consider mapping a group $B$ of weight blocks onto one PTC $A$.
Firstly, we can obtain the value range of weights at each position by extracting the first block and the last block, as the proposed sorting heuristic already sorts the weight values in ascending order.
Then, we can calculate the mapping deviation (MD) by mapping the $m$-th row of the group $B$ of weight blocks to the $n$-th row of PTC $A$ as follows,
{\small
\begin{align}
    &MD(B_{m}, A_{n})\\
    =& \sum_{i}^{k}\gamma_{i}^{+} |B_{mi, max}- A_{ni, max}| + \gamma^{-}_{i} |B_{mi, max} - A_{ni, max}|, \nonumber
\label{eq:MD_eq} 
\\
&\gamma_{i}^{+} =\left\{
    \begin{aligned}
        &1, \ B_{mi, max} > A_{ni, max} \\
        &0, \ \text{otherwise}
    \end{aligned}
    \right. \nonumber \\
& \gamma_{i}^{-} =\left\{
    \begin{aligned}
    &1, \ B_{mi, max} < A_{ni, max} \\
    &0, \ \text{otherwise}
    \end{aligned}
    \right.\nonumber
\end{align} 
}
where $k$ is the length of the $n$-th row of $A$, $W_{mi, max}$ and $W_{mi, min}$ refer to the maximum and minimum  value of weights in the $m$-th row and $i$-th column of weight blocks in $B$.
% , which represents the weight range.
Accordingly, $A_{ni, max}$ and $A_{ni, min}$ refer to the supported maximum and minimum transmission values at $A_{ni}$.
$\gamma_{i}^{+}$ and $\gamma^{-}$ indicate whether the range of weights exceeds the supported range.

Hence, to minimize the mapping deviation of $k$ rows by searching an optimized row order $\pi^{*}$, the re-mapping problem is defined as,
\begin{equation}
    \small
    \pi^{*} = \arg \min \sum_{r}^{k} MD(B_{\pi(r)}, A_{r}).
\end{equation}
This re-mapping problem can be viewed as a weighted bipartite matching problem with a minimum sum of edge costs.
Specifically, rows in weight blocks and PTC consists of the set $L$ of vertices and the set $R$ of vertices, respectively. 
The mapping deviation between $m$-th row in a set $B$ of weight blocks and $n$-th row of PTC, i.e., $MD(B_m, A_n)$, corresponds to the edge cost.
Thus, the optimized row order $\pi^{*}$ can be obtained by finding a perfect matching of minimum cost, which can be solved by Hungarian algorithm~\cite{NPC_Hungarian1955_kuhn}.
Note that our scheme tolerates aged PCM wires efficiently, where we reorder the rows for a group of weight blocks instead of reordering blocks one by one.

\iffalse
The rows in extract weight range matrix $W$ and PTC $A$ are a set $L$ of vertices and a set $R$ of vertices.
An edge $(i, j)\in E$ indicates the $i$-th row of $W$ is assigned to the $j$-th row in the PTC, associated with the edge cost $c_{ij}=RMD(W_i, A_j)$.
Thus our target is transformed to find a perfect matching of minimum cost where the cost of a matching $M$ is given by $c(M)=\sum_{(i,j)\in M} c_{ij}$ .
Hungarian algorithm is adopted to solve this problem such that we can obtain the optimal order $\pi^{*}$ in polynomial time.
\fi

\iffalse
In \cite{NP_DATE2017_chen}, the similar method is adopted to remap the rows of weight blocks onto RRAM crossbar. 
However, they need re-compute the swap order when mapping each weight block while our method chooses to remap once for a group of weight blocks with the shared swap order.
Thus, our globally row-reordering leads to stuck-at-faults tolerance in a highly efficient way.
\fi

\iffalse
Due to the limited endurance of PCM, over-utilization of PCM memory cells leads to the aging of inside PCM wires.
The phase state of aged PCM wires is complex and dynamic, leading to uncontrolled drifts away from expected values.
Without considering aging, the weights of NN model are usually directly mapped onto the transmission range of PCM memory cells in fresh state.
However, the existence of aged cells will introduce value variations to real mapped values, drifting them from desired values.
The inference accuracy of networks is very sensitive to the value variations, typically resulting in serious accuracy degradation.

As not all PCM wires inside single PCM memory cell wear out in the meanwhile, 
fixing PCM wires to known phase states before exceeding endurance can enable further utilization of aged PCM memory cells.
It is called that stuck-at-faults happen on these PCM memory cells.
% When some wires of PCM memory cells are tied to specific states, it is called that stuck-at-faults happen on the PCM memory cells. 
Different from previous definition of stuck-at-faults(SAF) \cite{NP_ASPDAC2019_Xia}, in this paper, stuck-at-faults of aged PCM memory cell refer to that a portion of PCM wires inside $n$-bit PCM memory cell is tied to specific states.

With stuck-at-faults, the upper bound and the lower bound of transmission levels may change in aged PCM memory cells.
For example, the max transmission level in both positive and negative decrease in Fig.~\ref{fig:StruckFaultMapDeviation} as a result of several PCM wires are stuck in both positive and negative PTC. 
However, the value range of a sequence of weights covers a wide range than supported transmission levels on aged PCM cell, resulting in map deviation.

to alleviate the mapping problem after aging, we take the map deviation into account when map groups of weight blocks to the PTCs in each layer.
We propose a global row reordering method to tolerate stuck-at-faults in an efficient way.
In the proposed method, we swap the rows of weight blocks $B$ assigned to the same PTC in the same sequence as their weights are constrained to be similar.
Because of the sort operations in the phase 2, the range of weights can be extracted by selecting the first block and the last block in the block sequence $B$, which we donate the weight range block as $W$.
Then, 
\fi

 \if
% \subsection{Problem formulation}
To implement inference tasks, reusing limited tensor cores for realizing large-scale matrix-matrix multiplication is needed, leading to frequent weight block mapping.
As the computation energy cost is very low in optical computing and the switching of PCM phase is excited by electrothermal-heating, the energy cost of weight mapping  is the main culprit.

The cost of inscribing weight value into PCM memory cells are determined by the difference between quantized levels of mapped values and pre-stored values.
Specifically, we need to consider the difference of levels in both positive and negative array.
The difference between quantized levels determines the number of PCM wires needed to be programmed between crystalline and amorphous phase.

{\small\begin{align}
    level(w)^{+} & =\left\{
\begin{aligned}
\texttt{Clip}( \texttt{Round}(\log_{t}(s|w|+\delta)), 0, 2^B-1), \ w \geq 0 \\
2^B-1, \ w < 0
\end{aligned}
\right.  \nonumber \\
level(w)^{-} & =\left\{
\begin{aligned}
2^B-1, \ w \geq 0 \\
\texttt{Clip}( \texttt{Round}(\log_{t}(s|w|+\delta)), 0, 2^B-1), \ w < 0
\end{aligned}
\right.
\label{eq:level_pos}
\end{align}}

Accordingly, we define the writing difference between two $B$-bit numbers $a$ and $b$ as

\begin{equation}
\small
    LD(a, b) = |Level(a)^{+} - Level(b)^{+}| + |Level(a)^{-} - Level(b)^{-}|
\end{equation}

Hence, 
the overall writing times when remapping block $B$ onto block $A$ can be computed as 

\begin{equation}
\small
    \mathcal{L}_{BML} = \sum_{c}^{C}\sum_{j}^{N^c}BMD(W_j^{c} - W_{ref}^{c})
\end{equation}
\begin{equation}
\small
\begin{aligned}
BLD(B, A) = \sum_{i}^{K}\sum_{j}^{K} (|Level(b_{ij})^{+} - Level(a_{ij})^{+}|& \\+ |Level(b_{ij})^{-} - Level(a_{ij})^{-}|&)
\end{aligned}
\end{equation}

{\small\begin{align}
    &\pi^{*} = \arg \min \sum_{i}^{p} \sum_{r}^{K} MD(W_{\pi(r)}, A(r)) \\ \nonumber
    \text{s.t.}~~& MD = \sum_{k}^{K}\gamma_{k}^{+} |W_{k, max}^{+} - A_{k, max}^{+}| + \gamma^{-} |W_{k, max}^{-} - A_{k, max}^{-}| \\ \nonumber
    & \gamma_{k}^{+} =\left\{
    \begin{aligned}
    1, \ W^{+}_{k, max} > A_{k, max}^{+} \\
    0, \ \text{otherwise}
    \end{aligned}
    \right.  \\ \nonumber
    & \gamma_{k}^{-} =\left\{
    \begin{aligned}
    1, \ W^{-}_{k, max} < A_{k, max}^{-} \\
    0, \ \text{otherwise}
    \end{aligned}
    \right.
\label{eq:level_pos}
\end{align}}

{\small\begin{align}
    \mathcal{L}_{BM} = \sum_{l}^{L}\sum_{g}^{G}\sum_{b}^{B}\sum_i^{K}\sum_j^{K}( &\lVert Level_{l,g, b,i,j}^{+} - Level_{l, g, ref}^{+}\rVert^2 \\ \nonumber
    &+ \lVert Level_{l,g, b,i,j}^{-} - Level_{l, g, ref}^{-}\rVert^2)
\end{align}}

Consider a weight matrix $W\in \mathbb{R}^{m\times n}$ in layer $l$.
Assume a single core can support $K\times K$ weight blocks such that the weight matrix $W$ can be partitioned into $p\times q$ sub-matrices.
Thus, for layer $i$, mapping of the weight blocks $B$ to hardware $H$ with a set $T$ of tiles $\mathcal{M}=\{m_{xy}\}$ is defined as

\begin{equation}
\small
    m_{xy} =\left\{
    \begin{aligned}
    &1, \ \text{if block $B_x \in B$ is mapped to tile $t_y \in T$} \\
    &0, \ \text{otherwise}
    \end{aligned}
    \right.
\end{equation}
And a block can map to exactly one tile such that $\sum_{y} m_{xy} = 1$.

In practical spatial acceleration of GEMM, specialized processing dataflows are designed to enable data reuse across different computation units, which reduce access cost to more expensive memory hierarchies in terms of energy and latency. 
The dataflow strategy also determine the mapping strategy $\mathcal{M}$. 

\textcolor{red}{why we need reuse data such that we only need to program the same input? one laser is enough?}
Without loss of generality, we leverages the data reusing as shown in Fig~\cite{fig:parallel_gemm}.
The weight blocks in same column in the partitioned weight matrix can share the same input data, while the partial sums are accumulated later.
In this regard, to reuse input data, it is desired to map those blocks belong to the same column to different tensor cores.
Hence, to simplify discussion, we consider a mapping scheme where we have enough $p$ tensor cores and each tensor core corresponds to a row of blocks.
In this regard, only one block of input data is needed to complete $p$ matrix-matrix multiplication.
For example, as shown in Fig~\ref{fig:parallel_gemm}, the dark blue weight blocks are programmed to different tensor cores and are multiplexed with dark green input data matrix.



We have the overall computing times on one specific tile $s$ as 
\begin{equation}
\small
    WT(t_s) = \sum_{B\in G_{y}}(WT(B, B_{pre})), G_{y} = {B_x} \ni m_{x,s}=1
\end{equation}

Thus, we have the writing times for each layer l as 
\begin{equation}
\small
    WT_{l} = \sum_{t_y \in T} \sum_{B\in G_y}(WT(B, B_{pre})), \ G_{y} = {B_x} \ni m^{l}_{x,y}=1 
\end{equation}

The optimization problem of our mapping-aware optimization is defined as 
\begin{equation}
    \small
    \label{eq:Objective}
    \begin{aligned}
    &\min(\sum_{l=1}^{L}WT_l),\\
    \text{s.t.}~~&WT_{l} = \!\!\sum_{t_y \in T} \!\sum_{B\in G^l_y}(WT(B, B_{pre})), \ G^{l}_{y} = {B^{l}_x} \ni m^{l}_{x,y}=1, \\
    & m^{l}_{x,y} = 1, \ \text{if block $B_{x}^{l} \in B^{l}$ is mapped to core $t_{y} \in T$}, \\
    &\sum_y m_{x, y}^{l} = 1, \ \forall x.
    \end{aligned}
\end{equation}
Without loss of generality, 
\fi

==> texlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
%\geometry{twoside=true, head=13pt,
%	paperwidth=8.5in, paperheight=11in,
%	includeheadfoot, columnsep=2pc,
%	top=35pt, bottom=65pt, 
%    left=45pt, right=45pt, 
%    %inner=54pt, outer=54pt,
%	marginparwidth=2pc,heightrounded
%}%
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cite}
\usepackage{cleveref}  % smart citation
%\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}
\sisetup{product-units = single}
% ==== Local new commands
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calS}{\mathcal{S}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
%\newcommand{\m}[1]{\mathbf{#1}}
%\newcommand{\mx}{\m{x}}
%\newcommand{\my}{\m{y}}
%\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}


==> texlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


\usepackage[noend]{algpseudocode}
%\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command
\usepackage{caption} 
\usepackage{subfig}

\usepackage{cleveref}                                      % smart



\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}

% ==== Local new commands
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calS}{\mathcal{S}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
%\newcommand{\m}[1]{\mathbf{#1}}
%\newcommand{\mx}{\m{x}}
%\newcommand{\my}{\m{y}}
%\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%




==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


